Learning Continuous Environment Fields via Implicit Functions

We propose a novel scene representation that encodes reaching distance -- the distance between any position in the scene to a goal along a feasible trajectory. We demonstrate that this environment field representation can directly guide the dynamic behaviors of agents in 2D mazes or 3D indoor scenes. Our environment field is a continuous representation and learned via a neural implicit function using discretely sampled training data. We showcase its application for agent navigation in 2D mazes, and human trajectory prediction in 3D indoor environments. To produce physically plausible and natural trajectories for humans, we additionally learn a generative model that predicts regions where humans commonly appear, and enforce the environment field to be defined within such regions. Extensive experiments demonstrate that the proposed method can generate both feasible and plausible trajectories efficiently and accurately.

==> 2.Introduction.tex <==
\section{Introduction}

% Problem definition
  % Path planing in robotics as well as real-world
Path planing is one of the most fundamental yet challenging problems in robotics and computer vision.
%
Given a scene environment and a target position within the scene, path planing aims at navigating an agent from its current location towards the target while avoiding collision with obstacles in the scene.
%
In the past few decades, numerous studies have been carried out to resolve this problem and can be classified into three categories: a) classical path planning algorithms such as Breath First Searching (BFS), Dijkstra's algorithm~\cite{dijkstra1959note} and the Fast Marching Method (FMM)~\cite{sethian1996fast,fmm_path}. b) sampling-based methods such as Rapidly Exploring Random Tree (RRT)~\cite{lavalle1998rapidly,lavalle2001rapidly,bry2011rapidly} or Probabilistic Roadmaps (PRM)~\cite{kavraki1996probabilistic,kavraki1998analysis}. c) and learning-based algorithms~\cite{tamar2016value,campero2020learning,maruan_18,chaplot2021differentiable}. 
%
Yet, path planing, especially when applied in realistic dynamically changing scenarios, is far from resolved.
%
% Motivation
    % Efficiency
    % Continuity
    
Two main challenges remain. First, existing path planing methods are not efficient for dynamically changing environments. For instance, classical and sampling-based path planning algorithms require running the algorithm for every new environment or goal position.
%
Though learning-based methods~\cite{tamar2016value,campero2020learning,maruan_18} are able to generalize to changing scenes during inference, they still predict each step sequentially. 
%
Most importantly, most existing path planing methods~\cite{sethian1996fast,tamar2016value,campero2020learning,maruan_18,chaplot2021differentiable} assume discrete environments (e.g., 2D mazes) and fail to flexibly search paths in continuous real-world scenarios (e.g., 3D indoor environment), where an agent may take an arbitrary size step at any direction.
%\XT{example to explain dynamic changing continuous scenes}

% Method
To resolve these issues, in this work, we propose an efficient learning-based path planing algorithm for continuous dynamically changing scenes.
%
At the core of the proposed method is a novel environment representation dubbed as the ``environment field''.
%
For each position in the scene, the environment field captures the ``reaching distance'' -- the distance from this position to a given goal location along a feasible trajectory.
%
During inference, given a learned environment field, we navigate an agent by repeatedly moving it to the next feasible location with the smallest reaching distance, until it reaches the goal.
%

Crucially, to apply the proposed environment field efficiently to real-world continuous scenes such as 3D rooms, we instantiate it as an implicit function~\cite{Park_2019_CVPR,disn_19,sitzmann2019siren,disn_19,Occupancy_Networks} due to two major benefits of implicit functions: a) Neural implicit functions can be generalized to arbitrary goal positions or even arbitrary scene environments, allowing the generalization to different environment fields given different goal positions or scenes using a single neural implicit function. During inference, the environment field values at multiple locations in the scene can be queried by a single fast network forward, enabling efficient trajectory prediction. b) The neural implicit function is able to learn continuous environment fields using discretely sampled training data and can be readily generalized to continuous environments such as 3D indoor scenes.
%
% Contribution Summary
  % Propose environment field
  % Implement via implicit functions
  % Showcase maze navigation & indoor path planing for humans
  
We showcase the application of the proposed environment field in both human trajectory planing in 3D indoor environments and agent navigation in 2D mazes and observe comparable if not better results than state-of-the-art methods.
%
To summarize, our contributions include:
\begin{itemize}
 \vspace{-2mm}
 \item We propose environment field -- a novel scene representation that facilitates direct guidance to dynamic agent behaviors in a scene.
 \vspace{-2mm}
 \item We learn the dense environment field using an implicit function such that it can be efficiently applied to path planing in continuous dynamically changing scenes.
 \vspace{-2mm}
 \item We showcase the application of the environment field in human trajectory planing in 3D indoor environments and agent navigation in general 2D mazes, where both feasible and plausible trajectories can be produced efficiently and accurately.
\end{itemize}

==> 2.Introduction_v2.tex <==
\vspace{-5mm}
\section{Introduction}
\vspace{-1mm}
\label{sec:introduction}
Scene understanding aims to analyze and interpret a given environment.
%
The past few years have witnessed tremendous success in scene understanding, including semantic segmentation~\citep{long2015fully,li2017fully}, 3D scene reconstruction~\citep{sitzmann2019siren,sitzmann2019srns}, and depth estimation~\citep{monodepth2}.
%
%While these methods successfully learn scene representations that can segment or reconstruct the scene, such models fail to provide direct feedback to control the behavior of agents or humans in the scene, which is essential to high-level tasks \SF{the followings are not typical high-level tasks, they are more like dynamic/embodied/human-centric tasks.} including agent navigation~\citep{tamar2016value,campero2020learning}, affordance modeling~\citep{CVPR2019_affordance3D,wang2017binge,PSI:2019,PLACE:3DV:2020} and human behavior prediction~\citep{caoHMP2020} within the scene. \SF{The above sentence does not make much sense. We should not require a segmentation network to do navigation. Should say models that can control behaviors of agents are not sufficiently explored.}
%While these methods successfully learn scene representations that can segment or reconstruct the scene, such models only focus on ``static'' scene attributes while ignoring its dynamic functioning.
%
%For instance, the layout of an environment could provide direct feedback to guide a human walking in the scene without colliding into objects.
These methods are further applied to various embodied tasks including agent navigation~\citep{tamar2016value,campero2020learning}, affordance modeling~\citep{CVPR2019_affordance3D,wang2017binge,PSI:2019,PLACE:3DV:2020} and dynamic human behaviors modeling~\cite{caoHMP2020}.
%
However, they only capture ``static'' attributes (e.g., segmentation, depths) of a scene while ignoring its ``dynamic'' functioning (e.g., direct control to agent behaviors), leading to limited performance especially in dynamic agent behavior modeling.
%
For instance, ~\cite{caoHMP2020} propose to model dynamic human behaviors by generating a plausible trajectory of humans in indoor environments. 
%
Nonetheless, by only utilizing static scene representations (i.e. images and depths) as conditional inputs, the learned model fails to fully exploit the dynamic functioning of the scene so that the length of the generated human trajectory is limited by the model capacity.
%

%
In this paper, we design a new scene representation that explores the \textit{dynamic} functioning of a given scene, so that it can directly guide the behaviors of agents in a scene, e.g., navigating an agent to reach a given goal from an arbitrary faraway position in a physically plausible manner. We name this new representation as the {\em environment field}.
%
For any position in the scene, the environment field represents the reaching distance -- the distance from this position to a given goal location along a feasible and plausible trajectory. \SF{Unlike transitional 2D/3D representation that encodes shapes and appearance, or probability of categories, the environment field captures the distance from this position to a given goal location along a feasible and plausible trajectory, allowing agents moving towards the goal in a simple gradient decent fashion} 
%
During inference, given a learned environment field, we navigate an agent by repeatedly moving it to the next location with the smallest reaching distance until it reaches the goal. \SF{Can be removed}


Analytically solving for this dense environment field for each position is computationally prohibitive. \SF{This motivation is too short and unclear.}
%
Instead, we leverage neural implicit functions~\citep{Park_2019_CVPR,disn_19,sitzmann2019siren,disn_19,Occupancy_Networks} to regress the reaching distance at each position. \SF{There is no causal relation between the 1st and the 2nd sentence: if the traditional way is not good enough, you can train a deep net like VIN. No need to use implicit.}
%
We use implicit functions to learn environment fields for several reasons.  
%
First, neural implicit functions allow the generalization to different environment fields given different goal positions or scenes using a single neural implicit function. 
%
Second, the neural implicit function is able to learn continuous environment fields using discretely sampled training data. 
%
Third, querying the reaching distance between any position and the goal only requires a fast network forward pass, enabling efficient trajectory prediction.

Although the geometric feasibility \SF{what is geometric feasibility?} is sufficient for agent navigation in simple scenes such as 2D mazes, affordance \SF{what is affordance?} is essential for complex scenarios such as predicting human trajectories in indoor environments.
%
For instance, although it is physically possible for humans to reach from one point to another by passing under a desk, such a trajectory is rarely taken by humans in the real world.
%
To enforce semantic \SF{why semantic?} plausibility of the environment field in indoor environments, we additionally propose the \SF{learn an} {\em accessible region} -- plausible regions for humans to appear in. 
%
We generate the accessible region for each scene by learning a variational auto-encoder and mark locations outside the accessible region as obstacles. \SF{This is done by learning a VAE to match the distribution of locations where people are presented, conditioned on a point cloud 3D scene}
%
The environment field is trained to discriminate the accessible region and obstacles so that it can guide humans to avoid collision with obstacles.
%so that humans will not be led to such locations by the environment field. 

We showcase the application of the proposed environment fields in both human trajectory modeling in 3D indoor environments as well as agent navigation in 2D mazes, and observe comparable if not better results than state-of-the-art methods.
%
The contributions of this work are:
%\vspace{-1mm}
%\begin{itemize}
\vspace{-1mm}
\begin{compactitem}
 \item We propose the environment field model -- a novel scene representation that facilitates direct guidance to dynamic agent behaviors in a scene.
% \vspace{-2mm}
 \item We learn dense environment fields using implicit functions that simultaneously guarantees geometric and semantic feasibility.
% \vspace{-2mm}
 \item We showcase the application of the environment fields in human trajectory prediction in 3D indoor environments and agent navigation in general 2D mazes, where both feasible and plausible trajectories can be produced efficiently and accurately.
\vspace{-4mm}
%\end{itemize}
\end{compactitem}

==> 2.Introduction_v3.tex <==
\vspace{-5mm}
\section{Introduction}
\vspace{-1mm}
\label{sec:introduction}
Scene understanding aims to analyze and interpret a given environment.
%
The past few years have witnessed tremendous success in scene understanding, including semantic segmentation~\citep{long2015fully,li2017fully}, 3D scene reconstruction~\citep{sitzmann2019siren,sitzmann2019srns}, and depth estimation~\citep{monodepth2}.
%
These methods are further applied to various embodied tasks including agent navigation~\citep{tamar2016value,campero2020learning}, affordance modeling~\citep{CVPR2019_affordance3D,wang2017binge,PSI:2019,PLACE:3DV:2020} and dynamic human behaviors modeling~\cite{caoHMP2020}.
%
However, existing scene representations only capture the ``static'' attributes (e.g. semantic or depth knowledge of a scene) while ignoring the ``dynamic'' functioning (e.g. direct control to agent behaviors based on the scene layout), leading to limited performance especially in dynamic agent behavior modeling. \SF{While existing scene representation mostly capture the static attributes, such as semantic categories or depth, few work explores representations that can describe the dynamic functioning, e.g., how an agent move within an indoor scene. Existing approaches (e.g.,~\cite{caoHMP2020}) usually learn the dynamic of agents, e.g., pose sequences, directly from those static attributes, e.g., depth maps, leading to limited performance.}
%
For instance, ~\cite{caoHMP2020} propose to model dynamic human behaviors by generating a human trajectory of fixed length in an indoor environment conditioned on rendered images and depths of a 3D room. \SF{no clue shows this work has limited performance.}
%
Nonetheless, the scene images and depths only capture local scene layout knowledge and fails to provide explicit control to the generated trajectories based on the entire scene layout. 
%
Thus, the learned model cannot fully capture the dynamic functioning of the scene and only predicts human trajectories of a short length.

To better model dynamic behaviors of agents within a scene, we argue that it is desirable to have a scene representation that captures the dynamic functioning of the scene and provides direct control to agent behaviors.
%
To this end, we propose a scene representation dubbed as the {\em environment field} that encodes the distance from any position to a given goal location along a feasible and plausible trajectory.
%
Given the environment field of a scene, an agent can navigate to reach a goal from any position by repeatedly moving to the next location with the smallest distance until it reaches the goal.

In order to provide direct control to guide an agent to reach a given goal from {\em any} location in the scene, a prerequisite property of the environment field is being continuous and densely covering the entire scene. 
%
Naively learning such a dense field requires ground truth distance annotation at any location in the scene, which is computationally prohibitive to collect.
%
To resolve this issue, we leverage neural implicit functions~\citep{Park_2019_CVPR,disn_19,sitzmann2019siren,disn_19,Occupancy_Networks} that can learn a continuous field using discretely sampled training data.
%
During inference, querying the reaching distance between any position and the goal only requires a fast network forward pass, enabling efficient trajectory prediction.
%
%

Furthermore, to enforce generated human trajectories to conform to common human behavior patterns, we additionally propose and learn the {\em accessible region} -- plausible regions for humans to appear in via a variational auto-encoder.
%
The environment field is trained to discriminate the accessible region and obstacles so that it can guide humans to avoid collision with obstacles.

We showcase the application of the proposed environment fields in both human trajectory modeling in 3D indoor environments as well as agent navigation in 2D mazes, and observe comparable if not better results than state-of-the-art methods.
%
The contributions of this work are:
%\vspace{-1mm}
%\begin{itemize}
\vspace{-1mm}
\begin{compactitem}
 \item We propose the environment field model -- a novel scene representation that facilitates direct guidance to dynamic agent behaviors in a scene.
% \vspace{-2mm}
 \item We learn dense environment fields using implicit functions that simultaneously guarantees geometric and semantic feasibility.
% \vspace{-2mm}
 \item We showcase the application of the environment fields in human trajectory prediction in 3D indoor environments and agent navigation in general 2D mazes, where both feasible and plausible trajectories can be produced efficiently and accurately.
\vspace{-4mm}
%\end{itemize}
\end{compactitem}
